Manipulable Semantic Components: a Computational Representation of Data Visualization Scenes

Various data visualization applications such as reverse engineering and interactive authoring require a vocabulary that describes the structure of visualization scenes and the procedure to manipulate them. A few scene abstractions have been proposed, but they are restricted to specific applications for a limited set of visualization types. A unified and expressive model of data visualization scenes for different applications has been missing. To fill this gap, we present Manipulable Semantic Components (MSC), a computational representation of data visualization scenes, to support applications in scene understanding and augmentation. MSC consists of two parts: a unified object model describing the structure of a visualization scene in terms of semantic components, and a set of operations to generate and modify the scene components. We demonstrate the benefits of MSC in three applications: visualization authoring, visualization deconstruction and reuse, and animation specification.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/8_discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}
% \bpstart{Expressiveness of Object Model} A computational representation of data visualization scenes needs to be expressive: it should describe the structure and procedure of diverse charts. Its expressiveness can be understood at both the theoretical and operational levels. At the theoretical level, the MSC object model essentially provides semantic labels to objects in a data visualization scene. 

% \todo{Summarize the results.}



% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \textbf{MSC} & \textbf{Chartreuse} & \textbf{\begin{tabular}[c]{@{}l@{}}Auto-Extraction\\of Extensible\\Timeline\end{tabular}} & \textbf{Charticulator} & \textbf{InfoMotion} & \textbf{\begin{tabular}[c]{@{}l@{}}Data\\Illustrator\end{tabular}} & \textbf{Bluefish} 
% & \textbf{CompositeVis} \\
% \hline
% mark & \begin{tabular}[c]{@{}l@{}}visual\\element\end{tabular} & mark & mark & \begin{tabular}[c]{@{}l@{}}visual\\element\end{tabular} & mark & element & \begin{tabular}[c]{@{}l@{}}graphical\\object\end{tabular} \\
% \hline
% data scope & \cross & \cross & \redcross & \cross & data scope & \cross & \cross \\
% \hline
% glyph & unit & \cross & glyph & \begin{tabular}[c]{@{}l@{}}repeating\\unit\end{tabular} & group & group & \begin{tabular}[c]{@{}l@{}}graphical\\object\end{tabular} \\
% \hline
% collection & \cross & layout & glyph & \begin{tabular}[c]{@{}l@{}}element\\groups\end{tabular} & collection & group & \begin{tabular}[c]{@{}l@{}}graphical\\object\end{tabular} \\
% \hline
% composite & \cross & layout & \begin{tabular}[c]{@{}l@{}}constraint-\\based\\layout\end{tabular} & \begin{tabular}[c]{@{}l@{}}freeform\\layout\end{tabular} & \begin{tabular}[c]{@{}l@{}}nested\\collection\end{tabular} & \begin{tabular}[c]{@{}l@{}}perceptual\\relation\end{tabular} & \begin{tabular}[c]{@{}l@{}}visual\\composition\end{tabular} \\
% \hline
% \begin{tabular}[c]{@{}l@{}}reference\\element\end{tabular} & \cross & \cross & \begin{tabular}[c]{@{}l@{}}axis,\\legend,\\coordinate\\system\end{tabular} & \cross & \begin{tabular}[c]{@{}l@{}}axes and\\legends\end{tabular} & \cross & \cross \\
% \hline
% annotation & \begin{tabular}[c]{@{}l@{}}embellish-\\ment\end{tabular} & annotation & \greenCheck & connectors & \cross & \begin{tabular}[c]{@{}l@{}}Element\\connected-\\ness,\\common\\region\end{tabular} & \cross \\
% \hline
% \begin{tabular}[c]{@{}l@{}}visual\\encoding\end{tabular} & \begin{tabular}[c]{@{}l@{}}visual\\element\end{tabular} & \begin{tabular}[c]{@{}l@{}}visual\\encoding\end{tabular} & visual & \cross & \greenCheck & \greenCheck & \cross \\
% \hline
% scale & \cross & scale & scale & \cross & \greenCheck & \cross & \cross \\
% \hline
% \begin{tabular}[c]{@{}l@{}}algorithmic\\layouts\end{tabular} & \begin{tabular}[c]{@{}l@{}}unit\\layout\end{tabular} & representation & \begin{tabular}[c]{@{}l@{}}constraint-\\based\\layout\end{tabular} & \begin{tabular}[c]{@{}l@{}}unit\\layout\end{tabular} & \cross & \cross & \begin{tabular}[c]{@{}l@{}}visual\\composition\end{tabular} \\
% \hline
% \begin{tabular}[c]{@{}l@{}}graphical\\constraints\end{tabular} & unit layout & \cross & \cross & \begin{tabular}[c]{@{}l@{}}unit\\layout\end{tabular} & \greenCheck & \begin{tabular}[c]{@{}l@{}}perceptual\\relation\end{tabular} & \cross \\
% \hline
% camera & \cross & \cross & \cross & \cross & \cross & \cross & \cross \\
% \hline
% \end{tabular}
% }
% \caption{}
% \label{table:component_comparison}
% \end{table*}



% At the operational level, Mascot.js supports the creation and manipulation of more than 60 unique data visualization designs, available at \url{https://mascot-vis.github.io/gallery.html}, covering commonly used chart types as well as more esoteric designs like cycle plot \cite{robbins_introduction_2008} and treemap bar chart. 

% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \textbf{MSC} & \textbf{Chartreuse} & \textbf{\begin{tabular}[c]{@{}l@{}}Auto-Extraction \\ of Extensible\\Timeline\end{tabular}} & \textbf{Charticulator} & \textbf{InfoMotion} & \textbf{Data Illustrator} & \textbf{Bluefish} \\
% \hline
% repeat & \cross & \cross & \greenCheck & \cross & \greenCheck & \greenCheck \\
% \hline
% divide & \cross & \cross & \cross & \cross & \greenCheck & \cross \\
% \hline
% densify & \cross & \cross & \cross & \cross & \cross & \cross \\
% \hline
% classify & \cross & \cross & \cross & \cross & \cross & \cross \\
% \hline
% repopulate & repeat & \greenCheck & \greenCheck & \cross & \cross & \cross \\
% \hline
% stratify & \cross & \cross & \cross & \cross & \cross & \cross \\
% \hline
% \begin{tabular}[c]{@{}l@{}}apply visual\\encoding\end{tabular} & morph, recolor & \greenCheck & \greenCheck & \cross & \greenCheck & \greenCheck \\
% \hline
% customize scale & \cross & \cross & \greenCheck & \cross & \greenCheck & \cross \\
% \hline
% \begin{tabular}[c]{@{}l@{}}set channel values\\directly\end{tabular} & fix & \cross & \greenCheck & \cross & \greenCheck & \greenCheck \\
% \hline
% apply layout & partition & \greenCheck & \greenCheck & \cross & \greenCheck & \greenCheck \\
% \hline
% \begin{tabular}[c]{@{}l@{}}update layout\\parameters\end{tabular} & \cross & \cross & \greenCheck & \cross & \greenCheck & \greenCheck \\
% \hline
% \begin{tabular}[c]{@{}l@{}}apply graphical\\constraints\end{tabular} & move & \cross & \cross & \cross & \greenCheck & \greenCheck \\
% \hline
% \begin{tabular}[c]{@{}l@{}}configure\\camera\end{tabular} & \cross & \cross & \cross & \cross & \cross & \cross \\
% \hline
% \end{tabular}}
% \caption{Comparison of scene abstraction operations in different frameworks.}
% \label{tab:operations}
% \end{table*}


% layering

% nested treemap/circle packing

% choropleth

% not focusing on statistical calculation etc. \todo{set visualizations? choropleth maps? unit visualizations}



% \todo{what about swapping x/y axis, changing a chart orientation? can be broken down into these operations.}

\bpstart{Implications on System Architecture} 
The operations in MSC can be broadly construed as constraints \cite{ren_charticulator_2018,vander_zanden_lessons_2001}:  for example, the generative operations, layout operations, and encoding-related operations are one-way dataflow constraints, while operations that apply affixation and alignment can be described as multiway constraints. Ideally, these constraints should be represented and solved in a reactive architecture: whenever the value of a variable (e.g., a component's channel) is changed, the architecture should automatically propagate the change and update the values of the other dependent variables. The current implementation of Mascot.js does not yet effectively support such reactive behaviors. In future work, we plan to investigate reactive architectures for MSC and constraint-solving methods to enable dynamic design-time manipulation (e.g., construction and editing of visual representations) and run-time interaction (e.g., interactive or animating behaviors). 

% Any visualization grammar needs to consider and make trade-offs between expressiveness, conciseness, extensibility, explainability and learnability. We discuss how \atlas fares along these dimensions by comparing it to three state-of-the-art grammars and toolkits: Vega-Lite~\cite{satyanarayan_vega-lite_2016}, Vega~\cite{noauthor_vega_2021} and D3\cite{bostock_d3_2011}.

\bpstart{Computational Representations for Deep Learning} MSC represents an initial step towards rethinking computational representations for data visualization. In fields like natural language processing, different computational representations such as distributed word representations, and sequence models for text data have enabled many applications such as information retrieval and content generation. In this paper, we considered a particular type of computational representation for three downstream tasks: authoring, deconstruction/reuse, and animation specification. We are interested in the viability of MSC as a foundation for future investigations on computational representations (e.g., vector-based embeddings or graph neural networks) that power deep learning techniques for additional downstream tasks. 

% can MSc lays the foundation for future investigations on computational models of data visualizations for deep learning applications. Code snippets as a representation, what are the implications of MSC as a foundation for deriving vector-based or graph-based representations? For instance, screen2vec, or graph4GUI. 

% In terms of static visualizations, the expressiveness of \atlas in its current form is comparable to that of Vega-Lite. \atlas supports most examples in Vega-Lite's gallery except maps, horizon graph, and visualizations with variable stroke widths. Meanwhile, the violin plot, radar plot, stellar chart and ridgeline plot are supported by \atlas but are missing from Vega-Lite's gallery. \atlas' graphics-centric approach also offers flexibility in creating nested visualizations with custom layouts (e.g., \href{https://atlas-vis.github.io/gallery.html#MultipleBarCharts}{multiple bar charts positioned by data} \cite{noauthor_atlas_nodate}) and infographics (e.g., \href{https://atlas-vis.github.io/gallery.html#DumbbellChart}{\cite{noauthor_atlas_nodate-1}} ). Further evaluation is needed to confirm if such designs can be created using Vega-Lite. 
% its capacity needs further evaluation \cc{$\leftarrow$ this sentense is arguable since \atlas also needs further evaluation}. 
% \atlas does not yet have built-in support for statistical abstractions, however it is possible to perform such calculations using JavaScript and visualize the results using \atlas. Vega-Lite goes beyond static charts and supports interactive behavior, which is currently absent in \atlas. 

% All the designs discussed so far can be created using D3 and Vega. In addition, these two libraries support more diverse examples such as tree and network visualizations. \atlas is thus less expressive than D3 and Vega, but it is more concise. Most of \atlas' examples require less than 30 lines of code, and 43 out of 50 examples in the current gallery are realized in no more than 20 lines of code. 

% To demonstrate \atlas's expressiveness, we take Vega-Lite's gallery as a benchmark set. Except for visualizations in categories of Maps, Advanced Calculations and Interactive, only 2 charts, \href{http://vega.github.io/vega-lite/examples/area_horizon.html}{the horizon graph} and \href{http://vega.github.io/vega-lite/examples/point_angle_windvector.html}{wind vector map}, cannot be reproduced by \atlas. Meanwhile, \href{https://atlas-vis.github.io/gallery.html#ViolinPlot}{the violin plot}, \href{https://atlas-vis.github.io/gallery.html#RadarChart}{radar chart} and \href{https://atlas-vis.github.io/gallery.html#StellarChart}{stellar chart} are missing in the gallery but supported in \atlas. Currently, \atlas doesn't support geographic charts, calculation abstractions (e.g., variable stroke width), and interaction, which are parts of our future works.

% \atlas addresses the extensibility issue through a graphics-centric approach, where users directly modify graphical objects in the scene graph. For example, a radar chart is composed by (1) creating a circle mark, (2) performing \densify operator to turn the circle into a polygon, and (3) binding the radial distance channel with data (Figure~\ref{fig:radarANDstellar}).  To create a stellar chart, which is arguably better than a radar chart \cite{morin-chasse_stellar_2021}, there is no need to introduce a new star mark. We can simply insert new vertices between each pair of vertices in the radar chart with a fixed radial distance (Figure~\ref{fig:radarANDstellar}). Similarly, to create a violin plot, no definition of a new violin mark is necessary. Users can \rc{densify} a rectangle to get an area mark and combine it with a box plot glyph. \atlas thus enables us to compose complex glyphs from primitive marks. 

% Instead of the JSON format and the end-to-end rendering process in Vega-Lite and Vega, \atlas defines its own visualization object model~(VOM) with the graphics-centric procedural grammar. Allowing the user to directly edit the VOM, \atlas enhances extensibility to some extent. 
% We present \href{https://atlas-vis.github.io/gallery.html#RadarChart}{the radar chart} and \href{https://atlas-vis.github.io/gallery.html#StellarChart}{stellar chart} to illustrate this point in Figure~\ref{fig:radarANDstellar}. 
% The radar chart is rendered through (1) creating a circle mark, (2) performing \densify operator to turn the circle into a polygon, and (3) binding the radial distance channel with data. Then, the stellar chart can be easily achieved by inserting new vertices between each pair of vertices in the radar chart with a fixed radial distance.





% Compared to D3, \atlas is more concise while less expressive in general. Most of \atlas’s examples require less than 30 lines of code, and 43 out of 50 examples are realized in no more than 20 lines of code. However, charts like \href{https://observablehq.com/@d3/chord-diagram}{the chord diagram} and \href{https://observablehq.com/@d3/collapsible-tree}{collapsible tree} cannot be handled in \atlas at present. 

% Besides, \atlas's VOM-based grammar differs from the DOM-based one in D3 fundamentally. 
% \atlas defines its own visualization object model~(VOM) based on the unified terminology from recent authoring tools \cite{satyanarayan_critical_2019}, while D3 relies on the document object model~(DOM). Whether the custom VOM or the DOM is more advantageous depends on context \cite{bostock_d3_2011}. For proficient web developers, leveraging the DOM as the scene graph abstraction allows them to use their prior knowledge; but for novices, learning the VOM may be easier than mastering the DOM and the associated technology stack including SVG and CSS. The custom VOM enables flexible rendering to either SVG or WebGL with the same code that constructs a visualization; while it is possible to use D3 to render visualizations to an HTML canvas, significant efforts are required from users. 

% Our grammar decouples visualization logic from rendering technologies, thus there is no prerequisite for DOM\&SVG knowledge which is essential for learning D3. More specifically, D3 is ``declarative" in terms of editing the DOM structure while Atlas is ``declarative" in the sense that users define and edit the VOM structure. It is worth noting that VOM is based on the semantic structure of the visualization, which could be visually learned without much domain knowledge. Thus, it is expected that \atlas's grammar won't lead to a steep learning curve and could be introduced to broader users.

% Finally, the step-by-step authoring process in \atlas 
% % decomposes the generalization of charts, 
% potentially makes learning and debugging easier since the user could review intermediate results and locate the problems. We acknowledge that this claim is speculative and needs to be validated through empirical studies.

% it's not yet clear enough whether the proposed benefits above hold valid. In our future works, one important step is to conduct a user study that focuses on the four dimensions.
